Critic as Lyapunov function (CALF): a model-free, stability-ensuring agent

This work presents and showcases a novel reinforcement learning agent called Critic As Lyapunov Function (CALF) which is model-free and ensures online environment, in other words, dynamical system stabilization. Online means that in each learning episode, the said environment is stabilized. This, as demonstrated in a case study with a mobile robot simulator, greatly improves the overall learning performance. The base actor-critic scheme of CALF is analogous to SARSA. The latter did not show any success in reaching the target in our studies. However, a modified version thereof, called SARSA-m here, did succeed in some learning scenarios. Still, CALF greatly outperformed the said approach. CALF was also demonstrated to improve a nominal stabilizer provided to it. In summary, the presented agent may be considered a viable approach to fusing classical control with reinforcement learning. Its concurrent approaches are mostly either offline or model-based, like, for instance, those that fuse model-predictive control into the agent.

==> input/intro.tex <==
Reinforcement learning is a control philosophy where, unlike the classical theory, the controller is learned (adapted) through the pure \textit{experience} \ie data generated from the system in some manner: via exploring a predefined region of the state space (so called \textit{tabular methods}), Monte-Carlo runs or even online \cite{Sutton2018ReinforcementL,Bertsekas2019Reinforcementl,Lewis2013Reinforcementl,Vrabie2012OptimalAdaptiv,Bouzy2006MonteCarloGo,Lazaric2007Reinforcementl,Vodopivec2017montecarlotre}.
Its applications range from robotics \cite{Kumar2016Optimalcontrol,Borno2013TrajectoryOpti,Tassa2012Synthesisstabi,Surmann2020DeepReinforcem,Akkaya2019Solvingrubiks} to games such as Go, chess, shogi (also known as Japanese chess) \cite{Silver2016Masteringgame,Silver2018generalreinfor}, and even complex video games such as StarCraft II \cite{Vinyals2019Grandmasterlev}.
Some variants of simple policy gradients \cite{Baxter2001Infinitehorizo,Kakade2001naturalpolicy,Peters2006Policygradient}, like REINFORCE, do not utilize practically anything from the classical control theory and are more akin to stochastic approximation, which is common in pure data science.
Other, more intricate methods use the so called actor-critic structure, which is much closer to control.
Actor manifests the controller itself, whereas the critic can be interpreted as a controller adaptation unit.
Nowadays, the actor and critic are usually implemented as neural nets.
Evidently, it is crucial to study how the net weights converge.
Results in this direction are numerous.
But, and what is more important from the control field standpoint, the closed-loop stability only relatively recently has been starting to attract attention.
We point out in this note that the closed-loop stability is crucial not only by itself, but it also affects the controller adaptation manifested by the critic.
%Attempts to guarantee stability under reinforcement learning were and are being made.
One research direction to guarantee stability under reinforcement learning uses the techniques of classical adaptive control, robustifying controls in particular.
The contribution of this work if two-fold: first, we indicate and study in a simulation the limitations of robustifying controls in reinforcement learning.
This should be taken into account by the researchers in stabilizing reinforcement learning taking the route of adaptive control.
Second, we provide a new stochastic analysis of the critic net convergence and point out at the role of the environment stability in it.
%We start first with an overview of stabilizing reinforcement learning.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{On stabilizing reinforcement learning}
\label{sub_stabrl}

Three general groups of approaches to stabilizing reinforcement learning can be formulated: shield-based reinforcement learning, fusion of model-predictive control and reinforcement learning and Lyapunov-based reinforcement learning.
% In this section we will overview these approaches and compare them to the proposed method. 
The first group of approaches suggests to directly discard unsafe actions via, generally speaking, a filter which, depending on the context, may be called a shield, an overseer, a supervisor etc.
These algorithms vary in the way of how exactly the shield checks actions for safety and issues an emergency solution.

The actual design of the shield may be as simple as human-based \ie manual \cite{Saunders2017TrialerrorTow}, or as complex as formal-logic based \cite{Tan2020DeductiveStabi,Platzer2008Keymaerahybrid,Platzer2009EuropeanTrain,Fulton2018Safereinforcem}.
Fusion with model-predictive control is active subfield in stabilizing reinforcement learning (see \eg \cite{Zanon2020SafeReinforcem,Zanon2019Practicalreinf,Zanon2022Stabilityconst,Koller2018LearningBased,Berkenkamp2017SafeModelbase,Berkenkamp2019Safeexploratio}).
It is no wonder since model-predictive control possesses such an established machinery for guaranteeing stability of the closed loop, such as terminal costs, terminal constraints, contraction tools etc.
Finally, the Lyapunov stability theory was recognized in reinforcement learning already by Perkins \& Barto \cite{Perkins2002LyapunovDesign,Perkins2001Lyapunovconstr}.
Advancements were made since \cite{Chow2018Lyapunovbased,Berkenkamp2017SafeModelbase}, although such approaches to stabilizing reinforcement learning were offline and required checking a Lyapunov decay property over a region in the state space during running the agent.
This is not always feasible in industrial applications, such as robotics.
To this Lyapunov-based stabilizing reinforcement learning, agent design based on stabilization techniques of adaptive control can be categorized (approaches can be traced back to the early 2010s \eg \cite{Zhang2011Datadrivenrob}).

An elaborate approach was suggested by \cite{vamvoudakis2015asymptotically}, whose elements found application in later works \eg \cite{Yang2019Provablyglobal,Wei2020DiscreteTimeI,Su2020DecentralizedE,Zhang2020RobustOptimal,Jha2019InitialExcitat,Kontoudis2019KinodynamicMot,Jha2018DirectAdaptivea,Luy2018Machinelearnin,Yang2020Safeintermitte,Shi2023SafeReinforcem}, some from the recent years.
The key idea was to use robustifying controls inspired by \cite{Polycarpou2003lineapproximat}.
In the next section, we overview this technique of stabilizing reinforcement learning by robustifying controls.
%Essentially, a Lyapunov function for the closed-loop system was suggested in \cite{vamvoudakis2015asymptotically}, as well as one for the actor's and one for critic's weights, based on the value function utilizing a special \textit{robustifying term} in the agent's policy.
%We give a synopsis of the work \cite{vamvoudakis2015asymptotically} in the next section.
%Then, we indicate a flaw in the respective stability analysis.
%It is stipulated that \cite{vamvoudakis2015asymptotically} erroneously followed the ideas of adaptive control by \cite{polycarpou2003line}.
%Implications for similar control schemes are discussed.

%The authors of \cite{vamvoudakis2015asymptotically} claimed to obtain a Lyapunov function for the closed-loop system, as well as for the actor's and critic's weights, based on the value function utilizing a special \textit{robustifying term} in the agent's policy.

%The work \cite{vamvoudakis2015asymptotically} can be roughly classified as Lyapunov-based stabilizing reinforcement learning and is, moreover, online.
%The authors of \cite{vamvoudakis2015asymptotically} claimed to obtain a Lyapunov function for the closed-loop system, as well as for the actor's and critic's weights, based on the value function utilizing a special \textit{robustifying term} in the agent's policy.
%Unfortunately, the respective mathematical derivations contain a serious flaw.
%We critically analyze it after a synopsis of the work \cite{vamvoudakis2015asymptotically} which we give in the next section.
%It is stipulated that Vamvoudakis et al. erroneously followed the ideas of adaptive control by \cite{polycarpou2003line}.
%In our view, the work \cite{vamvoudakis2015asymptotically} cannot be fixed in any way that could follow the claimed approach closely.
%Nevertheless, it is actively cited: refer \eg to \cite{wei2020ImpulsiveADP, su2020decentralized, zang2020robustNonlinear, Jha2019LTIsystems, KinodynamicVamvoudakis, jha2018LTIwithoutPEcondition, MLbasedMultipleAgentsNguen, YangVamSafe}.
%
%\red{ here} \cite{YangVamSafe} used a robustifying term
%
%Also, similar ideas can be traced back to \cite{zang2011robust}.
